Biased Average Position Estimates in Line and Bar Graphs: Underestimation, Overestimation, and Perceptual Pull

In visual depictions of data, position (i.e., the vertical height of a line or a bar) is believed to be the most precise way to encode information compared to other encodings (e.g., hue). Not only are other encodings less precise than position, but they can also be prone to systematic biases (e.g., color category boundaries can distort perceived differences between hues). By comparison, position's high level of precision may seem to protect it from such biases. In contrast, across three empirical studies, we show that while position may be a precise form of data encoding, it can also produce systematic biases in how values are visually encoded, at least for reports of average position across a short delay. In displays with a single line or a single set of bars, reports of average positions were significantly biased, such that line positions were underestimated and bar positions were overestimated. In displays with multiple data series (i.e., multiple lines and/or sets of bars), this systematic bias still persisted. We also observed an effect of "perceptual pull", where the average position estimate for each series was 'pulled' toward the other. These findings suggest that, although position may still be the most precise form of visual data encoding, it can also be systematically biased.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
last modified by Bernhard Finkbeiner, July 5, 2010

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored by
the IEEE Visualization & Graphics Technical Committee (VGTC).

The only conferences that use the 'journal' document option:
- IEEE Visualization Conference (Research and Application Papers Only)
- IEEE Information Visualization Conference (Research and Application
Papers Only)

It contains 13 files:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed,
                  somewhere in the TeX search path
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
sample.eps      - an image used by the example paper
sample.pdf      - its PDF version
template-journal*.pdf    - an example proper pdf output in default
                          conference mode, with and without teaser
CypressView.eps - teaser image
CypressView.pdf - its PDF version
makefile     - makefile including bibtex compilation and proper PDF
                generation

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We
suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create
a file called 'template.pdf'. Please make sure, that its layout is
identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process
manually.  Below are a list of available options that may be passed to
make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> ez_modeling.tex <==
%% MIXTURE MODELING %%
\section{Mixture Modeling}
We propose a simple perceptual mixture model to computationally quantify the strength of the perceptual pull exerted by other graphed data series onto the target data series. The basic idea of the model is that a compound stimulus generates independent percepts of both graphed data series (the target and the `non-target'), and the reported target estimate is thought to be a weighted combination of these two independent percepts. An ideal observer would have a weight associated with the target data series of 1 and a weight for the non-target data series of 0, indicating no influence of the irrelevant non-target on perception of the target. However, the perceptual pull phenomenon indicates that the weight associated with the target data series will be less than 1, due to influence from the non-target data series. 

The aim of this section is simply to assess the viability of this idea. As such, we develop the model based on the `top line, bottom bar' compound stimulus from Experiment 3. For the sake of illustration, suppose the top line is the target data series. To model the compound stimulus judgments, we proceed as follows:

\begin{enumerate}[noitemsep]
 \item Draw a random sample from the empirical distribution of single line estimation \textit{errors}, $X_{target}$.
 \item Draw a random sample from the empirical distribution of single bar estimation \textit{errors}, $X_{non-target}$.
 \item Draw a random \textit{pair} of true line and bar positions in the compound stimulus. Add the sampled single line and bar estimation errors to these true positions, giving the single data series percepts in a compound stimulus: $x^*_{target}$ and $x^*_{non-target}$.
 \item For a given weight associated with the target, compute the target line estimate in the compound stimulus: $y^*_{target} = w_{target} x^*_{target} + (1-w_{target}) x^*_{non-target}$.
 \item Repeat steps 1-4, $M$ times ($M = 10,000$ below). The resulting distribution may be regarded as a synthetic distribution of compound target estimates, $Y^*$.
 \item Fit the resulting distribution of compound target estimates with a kernel density. This is a kernel density approximation of the likelihood \cite{hartig:2011:Stochastic}.
 \item For each observed target estimate, $y_{i,obs}$ for $i=1,\ldots,N$, in the compound condition, compute the approximate likelihood by plugging it into the kernel density (using linear interpolation).
 \item Across all observations, compute the overall log-likelihood as $\mathcal{L}=\sum_{i=1}^{N} \text{ln } p(y_{i,obs}|\theta)$, where $\theta$ is the vector of model parameters (i.e. the weight associated with the target data series).
 \item Find the best-fitting weight parameter(s) through maximum likelihood estimation.\footnote{Note that the likelihood is stochastic, because it is based on weighted combinations of many random samples. We will deal with this issue below.}
\end{enumerate}

In modeling the data, we made a number of other necessary assumptions. First, we must assume that the only graphical elements influencing position estimations are the lines and bars on the display, and do not include other potentially biasing elements, such as the display frame. Second, all participants are assumed to behave in the same way. We have limited data for individual participants, so estimating model parameters at the level of the individual would involve sampling from a limited set of single data series estimates, which is likely to bias the approximate likelihood. Third, position estimation errors are assumed to be independent of the true positions of the graphed data series. That is, we sample from the single data series distributions pooled over the three different target means. As a result, any effects of the true position of the data series in a compound stimulus are not captured by the model. However, our data indicate that any such effects were very small ($\eta_{partial}$=.006; see section 6.2). Fourth, we assume that the weight associated with the target data series can depend on whether the target is the line (and the non-target is the bar) or whether the target is the bar (and the non-target is the line) (i.e., $w_{target=line} \neq w_{target=bar}$). Since we previously observed asymmetrical behaviors in average line and bar position estimations (underestimating lines and overestimating bars), this final assumption allows for asymmetric effects of non-target bars on target lines and vice versa. 

These assumptions mean that a given compound stimulus configuration (e.g., top line and bottom bars) is modeled with just two free parameters: the relevant target weight, which is allowed to depend on which data series is the target\footnote{It could be argued that the bandwidth of the kernel density is also a model parameter, but we simply adopted the default rule of thumb for a Gaussian kernel density \cite{silverman:2018:Density}.}. We make no assumptions about the nature of the single data series error distributions. The only assumption we make about the compound error distribution is that it is a weighted combination of the distributions of single data series errors. Overall underestimation or overestimation of the graphed data series is accounted for by the single data series error distributions, and the model captures how these overall shifts are `pulled' by competing, irrelevant data series.

For the test case here (top line and bottom bars), there were 1552 target estimates in a compound stimulus (773 line estimates; 779 bar estimates). Best fitting weight parameters were found using the standard `optim' function in R \cite{rLanguage}. Comparison with an optimal observer was performed by comparing the model fit with a 0-parameter model in which the weight associated with the target data series was set to 1 and the weight associated with non-target data to 0. For this optimal model, the distribution of compound target estimates is simply equivalent to the corresponding distribution of single target estimates. Model comparison was performed using the Akaike Information Criterion. To accommodate stochasticity in the likelihood function, we performed the optimization 50 times with random starting points for the weight parameter over the interval $[0.9, 1]$. We report the average AIC difference with the optimal model (mixture model AIC - optimal model; negative values indicate a better fit of the mixture model). Any variation in the log-likelihood for the mixture model stems from two sources: the best-fitting parameters may depend slightly on the randomly chosen starting values. However, even with the same (best-fitting) parameters, the model would return a slightly different likelihood due to the random sampling from the single data series error distributions. For the baseline model, only this second source of variation was considered.

\begin{figure}[t]
 \centering
 \includegraphics[width=8cm]{Anchoring_AIC.png}
 \caption{The mixture model of perceptual pull is suggested to be a good fit. In 50 iterations of optimization, only 4\% had positive AICs.}
 \label{fig:model_AIC}
\end{figure}

\begin{figure}[b!]
 \includegraphics[width=8.8cm]{Anchoring_ModelFit.png}
 \caption{Comparison of mean model fit and 95\% confidence intervals of model predictions (represented by \textit{purple lines}).}
 \label{fig:model_fit}
\end{figure}

For the 50 model fits conducted in this way, the average AIC difference was $-104$ (95\% highest density interval=$[-145, -22]$). Only 2 out of 50 model fits had positive AICs, as shown in Figure~\ref{fig:model_AIC}. The mean weight for the line target was $0.945, CI=[0.901, 0.990]$, and the mean weight for the bar target was $0.971, CI=[0.933, 0.989]$. These weights are clearly close to 1, but the 95\% highest density intervals do not include 1. We would expect the weights to be close to 1, because the perceptual pull effects are relatively subtle but reliable. This suggests that when participants viewed compound line-bar displays, they made average line position estimates by attributing 94.5\% weight to the actual line position and the remaining 5.5\% to the bars below the lines, on average. Participants made average bar position estimates by attributing 97.1\% weight to the actual bar positions and the remaining 2.9\% to the lines above, on average. Figure~\ref{fig:model_fit} illustrates the model fit compared to the observed data. 

This model isolates the unique contribution of perceptual pull from the irrelevant depiction of the second data series. When there were two data series present on the graph, participants were not able to completely filter out the irrelevant data series. As a result, their target position estimate reflected a weighted combination of the target and non-target positions, reflecting an effect of perceptual pull.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

